Attainable Knowledge and Omniscience

The paper investigates an evidence-based semantics for epistemic logics. It is shown that the properties of knowledge obtained from a potentially infinite body of evidence are described by modal logic S5. At the same time, the properties of knowledge obtained from only a finite subset of this body are described by modal logic S4. The main technical result is a sound and complete bi-modal logical system that describes properties of these two modalities and their interplay.

==> eptcsdata.tex <==
\providecommand{\firstpage}{251}
\providecommand{\publicationstatus}{J. Y. Halpern and A. Perea (Eds.): Theoretical Aspects \\
of Rationality and Knowledge 2021 (TARK 2021) \\
EPTCS 335, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.335.24}{10.4204/EPTCS.335.24}}
\pdfoutput=1

